Adaptive Learning of the Optimal Batch Size of SGD

Recent advances in the theoretical understanding of SGD led to a formula for the optimal batch size minimizing the number of effective data passes, i.e., the number of iterations times the batch size. However, this formula is of no practical value as it depends on the knowledge of the variance of the stochastic gradients evaluated at the optimum. In this paper we design a practical SGD method capable of learning the optimal batch size adaptively throughout its iterations for strongly convex and smooth functions. Our method does this provably, and in our experiments with synthetic and real data robustly exhibits nearly optimal behaviour; that is, it works as if the optimal batch size was known a-priori. Further, we generalize our method to several new batch strategies not considered in the literature before, including a sampling suitable for distributed implementations.

==> Sections/conclusion.tex <==
\section{Conclusion}

In this paper, We proposed a robust algorithm, which adaptively selects  batch sizes throughout training, that consistently performs almost as if we used SGD with optimal  batch size and theoretically grounded its convergence. Besides, we introduced generalized sampling strategies that are suitable for distributed optimization. We derived formulas for computing optimal  batch size, and empirically showed its precision.
% We employ an effective technique to efficiently utilize memory usage and avoid seeing non-sampled data-points.
The proposed algorithm can be viewed as an enhancement on SGD that is orthogonal to many other approaches (e.g., variance reduction). Thus, it might be possible to combine them in future work.


